Symbolic Execution Game Semantics

We present a framework for symbolically executing and model checking higher-order programs with external (open) methods. We focus on the client-library paradigm and in particular we aim to check libraries with respect to any definable client. We combine traditional symbolic execution techniques with operational game semantics to build a symbolic execution semantics that captures arbitrary external behaviour. We prove the symbolic semantics to be sound and complete. This yields a bounded technique by imposing bounds on the depth of recursion and callbacks. We provide an implementation of our technique in the K framework and showcase its performance on a custom benchmark based on higher-order coding errors such as reentrancy bugs.

==> S-A-comp2.tex <==
\section{Compositionality of Concrete Games -- take 2}

In the following sections, we prove compositionality of our concrete game semantics. We use a bisimulation argument similar to \cite{DBLP:journals/corr/MurawskiT16a}. We begin by defining bisimilarity for concrete configurations.

Given the transition systems $(\mathcal{S},\rho_0,\to,\mathcal{F})$ and $(\mathcal{S}',\rho_0',\to',\mathcal{F}')$, we say that a relation $R \subseteq \mathcal{S} \times \mathcal{S}'$ is a \boldemph{bisimulation} if for all $(x,x') \in R$:
\begin{itemize}
\item $x \in \mathcal{F}$ iff $x' \in \mathcal{F}'$;
\item if $x \to y$ then $x' \to' y'$ and $(y,y') \in R$;
\item if $x' \to' y'$ then $x \to y$ and $(y,y') \in R$.
\end{itemize}
We also say $x$ and $x'$ are \boldemph{bisimilar}, written $x \sim x'$, if $(x,x') \in R$ and $R$ is a bisimulation.

We then define a notion of compatibility for configurations. We say configurations $\rho \in L$ and $\rho' \in C$, where $L$ has no main body, are compatible ($\rho \asymp \rho'$) if:
\begin{itemize}
\item their stores are disjoint: $\refs(L) \cap \refs(C) = \varnothing$
\item $\rho$ closes and is closed by $\rho'$: $\pub = \abs'$ and $\pub' = \abs$
\item undisclosed names of $\rho$ do not occur in $\rho'$ and vice versa: $(\meths(L) \setminus (\abs \cup \pub)) \cap \meths(C) = \varnothing$
\item their evaluation stacks are compatible, written $\eval \asymp \eval'$, which means:
\begin{itemize}
\item $\eval = \eval'$; or
\item $\eval = l::m::\eval_1$ and $\eval' = m::E::\eval_1'$, and $\eval_1 \asymp \eval_1'$; or
\item $\eval = m::E::\eval_1$ and $\eval' = l::m::\eval_1'$, and $\eval_1 \asymp \eval_1'$.
\end{itemize}
\end{itemize}
Note that compatibility of evaluation stacks expects that compatible configurations are always of opposite polarity. This may seem questionable at first since general compositionality allows the client to have an environment of its own, independent of $L$, and thus requires games between the composed configurations--as two opponent configurations--and an external client. However, we assume $L$ and $C$ close each other, meaning that $C$ captures the whole environment and would include any external interactions as internal moves of $C$, since we aim only to model check $L$. With these definitions, we follow by defining different notions of composition.

\subsection{Semantic Composition}
Let $\rho_1,\rho_2,\rho_1',\rho_2'$ be game configurations. Suppose there is a library $L$ and a client $C$ such that $\rho_1 = (\eval_1,\dots)$ and $\rho_1' = (\eval_1',\dots)$ are configurations of $L$, and $\rho_2 = (\eval_2,\dots)$ and $\rho_2' = (\eval_2',\dots)$ are ones of $C$. Given $\rho_1'\asymp \rho_2'$ and $\rho_1 \asymp \rho_2$, the following rules define the semantic composition of two configurations.
\begin{align*}
{\begin{prooftree}
\Hypo{ \rho_1 \to \rho_1' }
\Hypo{ \rho_2' = \rho_2 }
\Infer2[ $\textsc{Int}_L$ ]
{ \rho_1 \semcomp \rho_2 \to \rho_1' \semcomp \rho_2' }
\end{prooftree}}
\quad
{\begin{prooftree}
\Hypo{ \rho_2 \to \rho_2' }
\Hypo{ \rho_1' = \rho_1 }
\Infer2[ $\textsc{Int}_C$ ]
{ \rho_1 \semcomp \rho_2 \to \rho_1' \semcomp \rho_2' }
\end{prooftree}}
\end{align*}
\begin{align*}
{\begin{prooftree}
\Hypo{ \rho_1 \xrightarrow{\mathtt{call }(m,v)} \rho_1' }
\Hypo{ \rho_2 \xrightarrow{\mathtt{call }({m},\hat{v})} \rho_2' }
\Infer2[ $\textsc{Call$_1$}$ ]
{ \rho_1 \semcomp \rho_2 \to \rho_1' \semcomp \rho_2'\{v/\hat v\} }
\end{prooftree}}
\quad
{\begin{prooftree}
\Hypo{ \rho_1 \xrightarrow{\mathtt{call }({m},\hat{v})} \rho_1' }
\Hypo{ \rho_2 \xrightarrow{\mathtt{call }(m,v)} \rho_2' }
\Infer2[ $\textsc{Call$_2$}$ ]
{ \rho_1 \semcomp \rho_2 \to \rho_1'\{v/\hat v\} \semcomp \rho_2' }
\end{prooftree}}
\end{align*}
\begin{align*}
{\begin{prooftree}
\Hypo{ \rho_1 \xrightarrow{\mathtt{ret }(m,v)} \rho_1' }
\Hypo{ \rho_2 \xrightarrow{\mathtt{ret }({m},\hat{v})} \rho_2' }
\Infer2[ $\textsc{Ret$_1$}$ ]
{ \rho_1 \semcomp \rho_2 \to \rho_1' \semcomp \rho_2'\{v/\hat v\} }
\end{prooftree}}
\quad
{\begin{prooftree}
\Hypo{ \rho_1 \xrightarrow{\mathtt{ret }({m},\hat{v})} \rho_1' }
\Hypo{ \rho_2 \xrightarrow{\mathtt{ret }(m,v)} \rho_2' }
\Infer2[ $\textsc{Ret$_2$}$ ]
{ \rho_1 \semcomp \rho_2 \to \rho_1'\{v/\hat v\} \semcomp \rho_2' }
\end{prooftree}}
\end{align*}
where $\rho'\{v/\hat v\}$ is the configuration we obtain if we replace the $E[\hat v]$ or $M\{\hat v/x\}$ that appears in term position of $\rho'$ with $E[v]$ or $M\{v/x\}$ respectively.

\subsection{Composite Semantics and Internal Composition}
We now introduce the notion of composing game configurations \boldemph{internally}, which occurs when merging two compatible game configurations into a single composite semantics configuration. We first refine the operational semantics and produce a \boldemph{composite semantics}. This is necessary, firstly, due to a mismatch in method names caused by the need to refresh methods passed as arguments in opponent moves. More precisely, in the semantic composition, an opponent move ${call}(m,v)$--where $v$ contains methods names--has all names in $v$ replaced with fresh ones. Meanwhile, with internally composed configurations, all actions should occur, likewise, internally as a term reduction, meaning that the equivalent call does not refresh the names in $v$. Secondly, there is an asymmetry between the bounds of the opponent and proponent configurations. Proponent configurations are bounded internally while opponent configurations have no internal bounds, and thus are only bounded when playing moves. This requires that we keep track of two pairs of bounds, one for each component, which may change at different rates.

With this in mind, to define the composite semantics, we extend the term configurations to obtain tuples of the following form:
\[ (M,R_1,R_2,S,k_1,k_2,l_1,l_2) \text{ for which we shall write } (M,\vec{R},S,\vec{k},\vec{l})\]
where $R_1$ and $R_2$ are the library and client methods respectively, such that $dom(R_1) \cap dom(R_2) = \varnothing$, $S$ is the combined store, and $k_1,l_1$ and $k_2,l_2$ are bounds managed by the library and client.
\cutout{, where we write $\nil_i$ when a component $k_i$ in $\vec{k}$ or $l_i$ in $\vec{l}$ is equal to $\nil$}
All operators tagged with $i$ will be operating on the $i$th component; e.g. $\vec{R}[m \mapsto M]_i$ states that $R_i[m \mapsto M]$ in $\vec{R}$. We also extend $M$ by tagging all method names (written $m^i$) as well as all lambda-abstractions (written $\lambda^i$) with $i\in\{1,2\}$ to show whether they are being called from the library (1) or the client (2). We write $M^i$ to be the term $M$ with all its methods and lambdas tagged with $i$. Evaluation contexts are also extended to mark methods which are being called from the opposite polarity:
\[ E ::= \dots \mid \evalbox{E}^i \mid \evaltag{E}{i,l}\]
Intuitively, $i$ is the component that is currently at a proponent configuration in the equivalent game semantics, while $l$ is the opponent bound for component $3-i$. This will be used particularly when evaluating a method call $m^i v$ when $m \nin dom(R_i)$. Applying these changes, we define the semantics for composite terms ($\compsemto$).
\cutout{, where neither $k_i$ or $l_i$ are $\nil$}
 \begin{flalign*}
 &(E[\assert(i)],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[()],\vec{R},S,\vec{k},\vec{l}) \quad (i \neq 0)\\
 &(E[!r],\vec{R},S,\vec{k},\vec{l}) \compsemto  (E[S(r)],\vec{R},S,\vec{k},\vec{l})\\
 &(E[r:=v],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[()],\vec{R},S[r\mapsto v],\vec{k},\vec{l})\\
 &(E[\pi_j\pair{v_1,v_2}],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[v_j],\vec{R},S,\vec{k},\vec{l})\\
 &(E[i_1 \oplus i_2],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[i],\vec{R},S,\vec{k},\vec{l})\quad (i=i_1\oplus i_2)\\
 &(E[\lambda^i x.M],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[m],\vec{R}[m\mapsto \lambda x.M]_i,S,\vec{k},\vec{l})\quad (m \not\in dom(\vec{R}))\\
 &(E[\ifm{i}{M_1}{M_0}],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[M_j],\vec{R},S,\vec{k},\vec{l})\quad (j = 1 \text{ iff } i \neq 0)\\
 &(E[\letm{x=v}{M}],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[M\{v/x\}],\vec{R},S,\vec{k},\vec{l})\\
 &(E[\letrec{f=\lambda^i x.M}{M'}],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[M'\{m/f\}],\vec{R}[m \mapsto \lambda x.M\{m/f\}]_i,S,\vec{k},\vec{l})\\
 &(E[m^i v],\vec{R},S,\vec{k} +_i 1,\vec{l}) \compsemto (E[\evalbox{M\{v/y\}^i}^i],\vec{R},S,\vec{k},\vec{l})\quad(R_i(m) = \lambda y.M)\\
 &(E[m^i v],\vec{R},S,\vec{k},\vec{l}+_{3-i}1) \compsemto (E[\evaltag{m^{3-i}v}{i,l}],\vec{R}',S,\vec{k},\vec{l}[l_i \mapsto l_0])\quad(R_{3-i}(m) = \lambda y.M)\\
 &(E[\evalbox{v}^i],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[v^i],\vec{R},S,\vec{k}+_i 1,\vec{l})\\
 &(E[\evaltag{v}{i,l}],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[v^i],\vec{R}',S,\vec{k},\vec{l}[l_{3-i} \mapsto l,l_i \mapsto last(E)])\\
 &\qquad \text{if $last(E)$ is defined,}\\
 &\qquad \text{and $last(E) = \hat{l}$ if $E = E_1[\evaltag{E_2}{j,\hat{l}}]$ provided $E_2$ has no tags $\evaltag{\bullet}{j',\hat{l}'}$}
 \end{flalign*}

We continue by defining the \boldemph{internal composition} of compatible configurations $\rho_1 \asymp \rho_2$. Consider $L$-configuration $\rho_1$ is and $C$-configuration $\rho_2$, we define the internal composition $\rho_1 \confcomp \rho_2$ to be a configuration in our new composite semantics by pattern matching on the configuration polarity and evaluation stacks according to the following rules. For clarity, we annotate opponent and proponent configurations with $o$ and $p$ respectively.

\paragraph{Initial Configuration:}
\begin{align*}
\rho_1 &= ([],-,R_1,S_1,\pub_1,\abs_1,k_0,l_0)_o\\
\rho_2 &= ([],M_0,R_2,S_2,\pub_2,\abs_2,k_0,-)_p\\
\rho_1 \confcomp \rho_2 &= (\evaltag{\bullet}{1,l_1}[M_0^2],R_1,R_2,S_1 \uplus S_2,k_0,k_0,l_0,l_0)
\end{align*}

\paragraph{Interim Configuration (case OP):}
\begin{align*}
\rho_1 &= (\eval_1,-,R_1,S_1,\pub_1,\abs_1,k_1,l_1)_o\\
\rho_2 &= (\eval_2,M,R_2,S_2,\pub_2,\abs_2,k_2,-)_p\\
\eval_1 &= ({m},E)::\eval_1' \quad \eval_2 = (m,l_2)::\eval_2'\\
\rho_1 \confcomp \rho_2 &= ((\eval_1' \confcomp \eval_2')[E^1[\evaltag{M^2}{1,l_2}]],R_1,R_2, S_1 \uplus S_2, k_1,k_2,l_1,l_2)
\end{align*}

\paragraph{Interim Configuration (case PO):}
\begin{align*}
\rho_1 &= (\eval_1,M,R_1,S_1,\pub_1,\abs_1,k_1,-)_p\\
\rho_2 &= (\eval_2,-,R_2,S_2,\pub_2,\abs_2,k_2,l_2)_o\\
\eval_1 &= (m,l_1)::\eval_1' \quad \eval_2 = ({m},E)::\eval_2'\\
\rho_1 \confcomp \rho_2 &= ((\eval_1' \confcomp \eval_2')[E^2[\evaltag{M^1}{2,l_1}]],R_1,R_2,S_1 \uplus S_2, k_1,k_2,l_1,l_2)
\end{align*}
where $m,\hat{m} \in \meths_{\theta_a,\theta_b}$ and $\hat{m}$ is fresh in both $\eval_1'$ and $\eval_2'$, and $\eval_1' \confcomp \eval_2'$ is a single evaluation context resulting from the composition of compatible stacks $\eval_1'$ and $\eval_2'$, which we define as follows:
\begin{align*}
\eval \confcomp \eval &= \bullet\\
(({m}',E)::\eval_1'') \confcomp ((m',l)::\eval_2'') &= (\eval_1'' \confcomp \eval_2'')[E^1[\evaltag{\bullet}{1,l}]]\\
((m',l)::\eval_1'') \confcomp (({m}',E)::\eval_2'') &= (\eval_1'' \confcomp \eval_2'')[E^2[\evaltag{\bullet}{2,l}]]
\end{align*}
Notice that there is only one case for initial configurations, and that is because the game must start from a configuration where $L$ is the opponent while $C$ is the proponent.

\subsection{Bisimilarity of Semantic and Internal Composition}
Lemma \ref{bisim} states that, given $L$ and $C$ configurations, it is possible to obtain the composite semantics ($\compsemto$) from the semantic composition of the corresponding compatible configurations, and vice versa.

{\lemma{\label{bisim}}{Given $\rho \asymp \rho'$ where $\rho$ is an $L$-configuration and $\rho'$ is a $C$-configuration, it is the case that $(\rho \semcomp \rho') \sim (\rho \confcomp \rho')$.}}

\begin{proof}
We want to show that $R = \{(\rho_1 \semcomp \rho_2, \rho_1 \confcomp \rho_2) \mid \rho_1 \asymp \rho_2\}$ is a bisimulation. Suppose $(\rho_1 \semcomp \rho_2, \rho_1 \confcomp \rho_2) \in R$. We begin with case analysis on the transitions available to the semantic composite. If $(\rho_1 \semcomp \rho_2) \to (\rho_1' \semcomp \rho_2')$, then $\rho_1' \asymp \rho_2'$. Now, by cases of the transitions, we prove that composite semantics can be obtained from the semantic composition.
\begin{enumerate}
\item If $(\rho_1 \semcomp \rho_2) \to (\rho_1' \semcomp \rho_2')$ is an ($\textsc{Int}_L$) move, then we have internal moves in the execution of $\rho_1$ up to $\rho_1'$. Since the composite semantics is concrete and, by construction, equivalent to operational semantics when no methods of opposite polarity are called, we can see that $(\rho_1 \confcomp \rho_2) \compsemto (\rho_1' \confcomp \rho_2)$.

\item If $(\rho_1 \semcomp \rho_2) \to (\rho_1' \semcomp \rho_2')$ is a ($\textsc{Call}_1$) move, then we have that $\rho_1 \xrightarrow{\mathtt{call}(m,v)} \rho_1'$ and $\rho_2 \xrightarrow{\mathtt{call}(\hat{m},\hat{v})} \rho_2'$. We thus know $m$ is defined in $R_1$, so we have the following semantics for $\rho_1$ and $\rho_2$ where the evaluation stacks are not equal:
\begin{align*}
&(\eval_1,-,R_1,S_1,\pub_1,\abs_1,k_1,l_1)_o\\
&\quad \xrightarrow{\mathtt{call}(m,v)}(l_1-1::m::\eval_1,mv,R_1,S_1,\pub_1,\abs_1',k_1,-)_p\\
&(\eval_2, E[\hat m\hat v], R_2, S_2, \pub_2, \abs_2, k_2, -)_p\\
&\quad \xrightarrow{\mathtt{call}(\hat m,\hat v)}(\hat m::E::\eval_2,-,R_2',S_2,\pub_2',\abs_2,k_2,l_0)_o
\end{align*}
Assuming $v$ contains $n$ names $\meths(v) = \{m_1, \dots, m_n\}$, we know that $v = \hat v\{m_i/\hat m_i\}$ for each name $\hat m_i \in\meths(\hat v)$ where $1 \leq i \leq n$ and all names $\hat m_i$ are distinct and fresh in $dom(R_1) \cup dom(R_2)$. We thus have:
\begin{align*}
&\rho_1 \confcomp \rho_2 = ((\eval_1 \confcomp \eval_2)[\evaltag{E^2[\hat m^2\hat v]}{1,l_2}],\vec{R},S_1 \cup S_2,\vec{k},\vec{l}) \\
&\rho_1' \confcomp \rho_2' = ((\eval_1 \confcomp \eval_2)[\evaltag{E^2[\evaltag{m^1v}{2,l_1-1}]}{1,l_2}],\vec{R},S_1 \cup S_2,\vec{k},\vec{l}[l_2\mapsto l_0]-_1 1)
\end{align*}
Evaluating $\rho_1 \confcomp \rho_2$ with the composite semantics we have:
\begin{align*}
&((\eval_1 \confcomp \eval_2)[\evaltag{E^2[m^2v]}{1,l_2}],\vec{R},S_1 \cup S_2,\vec{k},\vec{l})\\
&\compsemto ((\eval_1 \confcomp \eval_2)[\evaltag{E^2[\evaltag{m^1 \hat{v}}{2,l_1-1}]}{1,l_2}],\vec{R},S_1 \cup S_2,\vec{k},\vec{l}[l_2\mapsto l_0]-_{1}1)
\end{align*}
Since $(\eval_1 \confcomp \eval_2)$ wraps $m^2v$ with substitutions that rename all $\hat{m}$ with $m$ that appear in the evaluation stacks, we know $(\eval_1 \confcomp \eval_2)[\hat m \hat v] = (\eval_1 \confcomp \eval_2)[m v]$ since $\eval_1 \confcomp \eval_2$ contain all names that have been passed so far.\todo{not true, the stack could evaluate, but names added to $\pub$ and $\abs$. We need to get names from there. Maybe we can say that all names in $\pub_1$ are used until a combination works?} We thus have that $(\rho_1 \confcomp \rho_2) \compsemto (\rho_1' \confcomp \rho_2')$. In addition, we can observe that the case for equal evaluation stacks is proven by substituting the initial stacks with equal ones, which results in an empty evaluation context. Similarly, the dual case ($\textsc{Call}_2$), where $m$ is defined in $R_2$, is identical but with polarities swapped--i.e. shown by the polar complement of $(\rho_1 \confcomp \rho_2) \compsemto (\rho_1' \confcomp \rho_2')$.

\item If $(\rho_1 \semcomp \rho_2) \to (\rho_1' \semcomp \rho_2')$ is a ($\textsc{Ret}_1$) move, then we have that $\rho_1 \xrightarrow{\mathtt{ret}(m,v')} \rho_1'$ and $\rho_2 \xrightarrow{\mathtt{ret}(m,v')} \rho_2'$. As with the \textsc{Call} case,  if $m \in dom(R_2)$ and stacks are not equal, we have:
\begin{align*}
&(m::E::\eval_1, - , R_1,S_1, \pub_1, \abs_1, k_1, l_1)_o\\
&\quad \xrightarrow{\mathtt{ret}(m,v')}(\eval_1, E[v'],R_1,S_1,\pub_1,\abs_1', k_1, -)_p\\
&(l_2::m::\eval_2,v,R_2,S_2,\pub_2,\abs_2,k_2,-)_p\\
&\quad \xrightarrow{\mathtt{ret}(m,v')}(\eval_2, - , R_2',S_2, \pub_2', \abs_2, k_2, l_2)_o
\end{align*}
where $R_2' = R_2[m_i' \mapsto \lambda x. m_i x]$ for every $m_i$ in $v'$. Here, we have two cases: $\eval_1 = \eval_2$, and otherwise. We start with the case where $\eval_1 \neq \eval_2$, since the opposite case is a simpler version of it. Again, we have the following composite configurations:
\begin{align*}
&\rho_1 \confcomp \rho_2 = ((\eval_1 \confcomp \eval_2)[E^1[\evaltag{v^2}{1,l_2}]],\vec{R},S_1 \cup S_2,\vec{k},\vec{l})\\
&\rho_1' \confcomp \rho_2' = ((\eval_1' \confcomp \eval_2')[E'^2[\evaltag{E^1[v'^1]}{2,l_1'}]],\\
&\qquad \qquad \quad \vec{R}[m_i'\mapsto \lambda x.m_i x]_2,S_1 \cup S_2,\vec{k},l_1',l_2)
\end{align*}
where $\eval_1 = l_1'::m'::\eval_1'$ and $\eval_2 = m'::E'::\eval_2$.
	
Now, from the composite semantics, we have:
\begin{align*}
&((\eval_1 \confcomp \eval_2)[E^1[\evaltag{v^2}{1,l_2}]],\vec{R},S_1 \cup S_2,\vec{k},\vec{l})\\
&\compsemto ((\eval_1 \confcomp \eval_2)[E^1[\hat{v}^1]],\vec{R}',S_1 \cup S_2,\vec{k},last((\eval_1 \confcomp \eval_2)[E^1[\bullet]]),l_2)\\
&~= ((\eval_1' \confcomp \eval_2')[E'^2[\evaltag{E^1[\hat{v}^1]}{2,l_1'}]],\vec{R}',S_1 \cup S_2,\vec{k},l_1',l_2)
\end{align*}

We can observe that $last(E) = l_1'$ since $E$ comes directly from the evaluation stack and is, thus, untagged, and the top-most bound is $l_1'$ since 
\[(\eval_1' \confcomp \eval_2')[E'^2[\evaltag{E^1[\bullet]}{2,l_1'}]] = (\eval_1 \confcomp \eval_2)[E^1[\bullet]]\]

In addition, we know $\vec{R}' = \vec{R}[m_i' \mapsto \lambda x.m_i x]$, and $v' = \hat{v}$ by determinism. Finally, we have that $k_2 = k_2'$ when returning a value since, from Lemma~\ref{kbounds}, $k$ must always increase back to its original value after evaluating a method call.

We thus have $(\rho_1 \confcomp \rho_2) \compsemto (\rho_1' \confcomp \rho_2')$. As previously, the case for empty stacks is a simpler version of this, while the dual case (2) is the polar complement of the configurations.
\end{enumerate}
	
Having shown that external composition produces composite semantics transitions, we continue with the other direction of the argument, which aims to show that the external composition can be produced from composite semantics transitions. We now derive the corresponding semantic compositions by case analysis on the composite semantics rules.
\begin{enumerate}
\item If we have an untagged transition, or one where the redex involves no names of opposite polarity being called, then we have an exact correspondence with internal moves, since the composite semantics are identical to the operational semantics on closed terms.

\item If the transition involves a method called from an opposite polarity, we have a transition of the form
\[(E[m^i v],\dots,\vec{l}) \compsemto (E[\evaltag{m^{3-i} v'}{i,l_{3-i}-1}],\dots,\vec{l}[l_i \mapsto l_0]-_{3-i}1)\]
which corresponds to evaluating the semantics on an initial configuration $\rho_1 \confcomp \rho_2$ with the following cases:
\begin{enumerate}
\item for an OP configuration, we have the following: 
\[\rho_1 = (\eval_1, -, R_1, S_1, k_1, l_1)_o\] 
\[\rho_2 = (\eval_2, E[m v], R_2, S_2, k_2, -)_p\]
where $\eval_1 = m'::E'::\eval_1'$ and $\eval_2 = l_2::m'::\eval_2'$. Let us set $E[m^i v] = (\eval_1' \confcomp \eval_2')[E'^1[\evaltag{M^2}{1,l_2}]]$ and $M^2 = E''[m^i v]$, where $m \nin R_2$, $i=2$, and $E''$ is untagged. We therefore have:
\begin{align*}
&((\eval_1' \confcomp \eval_2')[E'^1[\evaltag{M^2}{1,l_2}]],\vec{R},S_1 \cup S_2,\vec{k},\vec{l})\\
&\compsemto (E[\evaltag{m^{1} v'}{2,l_1-1}],\vec{R'},S_1 \cup S_2,\vec{k},\vec{l}[l_2 \mapsto l_0] -_1 1)
\end{align*}
We now want to show that semantically composing the configurations results in an equivalent transition $\rho_1 \semcomp \rho_2 \to \rho_1' \semcomp \rho_2'$. Since this is a $\textsc{Call}$ move, we know that $\rho_1 \xrightarrow{\mathtt{call}(m,v')}\rho_1'$ and $\rho_2 \xrightarrow{\mathtt{call}(m,v')}\rho_2'$. Evaluating those transitions, we have that
\[\rho_1' = (l_1 - 1::m::\eval_1,m v', \dots, k_1, -)_o\]
\[\rho_2' = (m::E''::\eval_2, -, \dots, k_2, l_0)_p\]
which, when syntactically composed, form the configuration 
\[((\eval_1 \confcomp \eval_2)[E''^2[\evaltag{(m v')^1}{2,l_1-1}]], \vec{R'}, S_1 \cup S_2, \vec{k}, \vec{l}[l_2 \mapsto l_0] -_1 1)\]
We can observe that the resulting configurations are equivalent since $E'' = E''^2$, which follows from $E''[m^i v] = M^2$. Additionally, since
\[(\eval_1' \confcomp \eval_2')[E'^1[\evaltag{E''^2[\bullet]}{1,l_2}]] = (\eval_1 \confcomp \eval_2)[E''^2[\evaltag{\bullet}{2,l_1-1}]]\]
it suffices to show $(m v')^1 = m^1 v'$, particularly that $v' = v'^1$. Now, since the composite semantics ensures that $v'$ will be tagged with $1$ when called from a method $m^1$, as it reduces to $M\{v'/y\}^1$, we have that $v' = v'^1$, meaning that the transitions are equal.
			
\item for a PO configuration, the polar complement of case (a) suffices.
			
\item for an initial configuration OP, we have a simpler version of case (a) where the evaluation stacks are equal, resulting in an empty evaluation context $\eval_1' \confcomp \eval_2' = \bullet$.
\end{enumerate}
		
\item If the transition involves a tagged value and is of the form
\begin{align*}
&(E[\evaltag{v}{i,l}],\vec{R},S_1 \cup S_2,\vec{k},\vec{l}) \\
&\compsemto (E[v'^{i}],\vec{R'},S_1 \cup S_2,\vec{k},\vec{l}[l_{3-i}\mapsto l, l_i \mapsto last(E)])
\end{align*}
then we want to show an equivalence to a \textsc{Ret} move in the semantic composite. As with case (2), we start by defining this transition as the syntactic composite transition $(\rho_1 \confcomp \rho_2) \compsemto (\rho_1' \confcomp \rho_2')$. Then, by case analysis on $\rho_1 \confcomp \rho_2$:
\begin{enumerate}
\item for an OP configuration, we have the following:
\[\rho_1 = (\eval_1, -, R_1,S_1, k_1, l_1)_o\] 
\[\rho_2 = (\eval_2, v, R_2,S_2, k_2, -)_p\]
where $\eval_1 = m::E'::\eval_1'$ and $\eval_2 = l_2::m::\eval_2'$. Let $E[v] = (\eval_1' \confcomp \eval_2')[E'^1[\evaltag{v^2}{1,l_2}]]$. We thus have:
\begin{align*}
&(E[\evaltag{v^2}{1,l_2}],\vec{R},S_1 \cup S_2,\vec{k},\vec{l})\compsemto(E[v'^1],\vec{R'},S_1 \cup S_2,\vec{k},last(E),l_2)
\end{align*}
We then show that semantic composition produces an equivalent transition $\rho_1 \semcomp \rho_2 \to \rho_1' \semcomp \rho_2'$. Given we have a \textsc{Ret} move, we know that $\rho_1 \xrightarrow{\mathtt{ret}(m,v')} \rho_1'$ and $\rho_2 \xrightarrow{\mathtt{ret}(m,v')} \rho_2'$, such that:
\[\rho_1' = (\eval_1', E'[v'], \dots, k_1, -)_p\]
\[\rho_2' = (\eval_2', -, \dots, k_2, l_2)_o\]
where $\eval_1' = l_1'::m'::\eval_1''$ and $\eval_2' = m'::E''::\eval_2''$. Internally composing these resulting configurations, we have:
\[((\eval_1'' \confcomp \eval_2'')[E''[\evaltag{E'^1[v'^1]}{2,l_1'}]], \vec{R'}, S_1 \cup S_2, \vec{k}, l_1',l_2)\]
Since $(\eval_1'' \confcomp \eval_2'')[E''[\evaltag{\bullet}{2,l_1'}]] = (\eval_1' \confcomp \eval_2')[\bullet]$, we have that $(\eval_1' \confcomp \eval_2')[E'^1[v'^1]]$, from which we have $(\eval_1'' \confcomp \eval_2'')[E''[\evaltag{E'^1[v'^1]}{2,l_1'}]] = E[v'^1]$, and that $last(E) = l_1'$ since $E_1'$ is untagged. Thus, the transition produces the composition.
			
\item for a PO configuration, we have the polar complement of (a) as previously.
			
\item for an initial OP configuration, we again have a simplification of (a), where the evaluation stacks are equal and the resulting evaluation context is empty.
\end{enumerate}		
\end{enumerate}
	
With this, we are done showing the equivalence of transitions. Lastly, we can observe that $\rho$ is final iff $\rho'$ is final since they are both leaf nodes generated by equivalent terminal rules. We therefore have $(\rho \semcomp \rho') \sim (\rho \confcomp \rho')$.
\end{proof}
	
\subsection{Syntactic Composition and Compositionality}
To prove compositionality of our game semantics, we want to show that the desired notion of syntactic composition can be obtained from semantic counterpart and vice versa. Now that we have bisimilarity between semantic and internal composition, we only need to show that internal composition is related to syntactic composition under some notion of equivalence. 

\todo{this paragraph might go}
First, we define the desired notion of syntactic composition. Let $L$ be a library and $C$ be a client such that $L$ and $C$ close each other. We define the notion of syntactic composition as a kind of syntactical concatenation with hiding. More precisely, given a library $X$ of the form $X = D;B$ where $D$ and $B$ are the method declarations and blocks respectively of the following form.
\begin{align*}
D &::= D;D \mid \mathtt{abstract}~m \mid \mathtt{public}~m \\
B &::= B;B \mid \lambda x.M \mid r := \lambda x.M \mid r:= i
\end{align*}
We define $\check{D}$ to be $D$ with all $\mathtt{abstract}$ declarations removed. With this, we say $L\syncomp C = \check{D}_L ; \check{D}_C ; B_L ; B_C$ is the \boldemph{syntactic composition} of $L = D_L;B_L$ and $C = D_C;B_C$, written $L \syncomp C$ . In other words, $L\syncomp C$ is the concatenation of $L$ and $C$ where all abstract method declarations are hidden.

\todo{this paragraph might go}
To define our desired notion of equivalence between syntactic and internal composites we use two different simulations: (1) one from the composite semantics to the syntactic composition, and (2) one in the opposite direction. In Lemma~\ref{simsim}, we define this notion of equivalence instead of attempting a proof of bisimilarity because the game semantics introduces an opponent bound that causes a difference in the length of the transition sequences. In other words, given the $L$ and $C$ starting configurations $\rho_0$ and $\rho_0'$, the semantics of $L\syncomp C$ defines a starting configuration $\check{\rho_0}$ with bound $\check{k}_0$, while the internal composite $\rho_0 \confcomp \rho_0'$ has bounds $\pair{k_0,k_0,l_0,l_0}$. This is a mismatch that cannot be resolved to prove bisimilarity as there is no single relation $R$ that can match $\check{\rho_0}$ with $\rho_0 \confcomp \rho_0'$ stepwise. Instead, we define $F$ and $G$ to relate $\pair{\vec{k}_0,\vec{l}_0}$ to $\check{k}_0$ and conversely. This way we have simulations in terms of $F$ and $G$ that do (1) and (2) separately. Intuitively, this means that, if the semantic composite reaches a bug with bounds $\pair{k_0,k_0,l_0,l_0}$, then the bug exists in the syntactic composite within $F(\vec{k}_0,\vec{l}_0)$, while any bug in the syntactic composite within $\check{k}_0$ will be found by the semantic composite within $G(\check{k}_0)$.

\todo{this paragraph might go later}
We proceed with some definitions that we will be using. Given a library $L$ and a client $C$ that close each other, if $(L \syncomp C) \xtwoheadrightarrow{lib} (\varepsilon,\check{R_0},\check{S_0})$, then let $\check{\rho_0} = (M_0,\check{R_0},\check{S_0},\check{k}_0)$, where $\check{R_0}(m_0) = \lambda().M_0$ and $m_0$ is the main method of $C$. Additionally, if $L \xrightarrow{lib} (\varepsilon,R_0,S_0,\pub_0,\abs_0)$ and $C \xrightarrow{lib} (\varepsilon,R_0',S_0',\pub_0',\abs_0')$ with the extended library semantics used in the symbolic setting, then let $\rho_0 = ([],-,R_0,S_0,\pub_0,\abs_0,k_0,l_0)_o$ and $\rho_0' = ([],M_0,R_0',S_0',\pub_0',\abs_0',k_0,-)_p$ be the starting configurations of $L$ and $C$ respectively. We thus define the semantics of $L \confcomp C$ as the transition sequence produced by the composite semantics starting from configuration $\rho_0 \confcomp \rho_0' = (M_0,\vec{R}_0,S_0 \cup S_0',\vec{k}_0,\vec{l}_0)$. We can also observe that $\check{R_0} \setminus R_0 = R_0'$ and $\check{S_0} \setminus S_0 = S_0'$, since $L$ and $C$ close each other, and $\rho_0$ and $\rho_0'$ contain all the method definitions and assignments available in each component respectively. As such, we define $\check{\rho_0}$ to be the syntactic composite of the starting configurations $\rho_0 \syncomp \rho_0' = (M_0,R_0 \cup R_0',S_0 \cup S_0',\check{k}_0)$, where $\check{k}_0 = F(\vec{k}_0,\vec{l}_0)$ and all polarity tags are removed. We can thus define the general translation from internal to syntactic composites by translating from the composite semantics to the equivalent operational semantics. This is
$\chi^\circ = (\rho_1 \syncomp \rho_2) = (M,R_1 \cup R_2,S,k_1 + k_2)$
where $\chi = (\rho_1 \confcomp \rho_2) = (M,\vec{R},S,\vec{k},\vec{l})$. \todo{define $\sem{L}_{k,l}$ to be the game semantics of $L$}

\bigskip\noindent
{\textbf{Theorem~\ref{simsim} (Compositionality)}~~{\em For any library $L$ and compatible client $C$, the following are equivalent.
\begin{enumerate}
\item There exists a bound $k$ such that $(L \syncomp C)$ with $k$ terminates with $\chi$.
\item There exist traces $\tau \in \sem{L}$ and $\tau^\bot \in \sem{C}$, and some bounds $k_1,k_2,l_1,l_2$, such that $\sem{L}_{k_1,l_1}$ terminates with $\chi$ by playing the moves in $\tau$.
\end{enumerate}
where $\chi$ is a configuration holding a term $v$ or $\assert(0)$.}
\begin{proof}
We have a case for each direction.
\paragraph{\bf $(1 \implies 2)$:}
\begin{enumerate}
	\item Consider $L\syncomp C$ with bound $k$ that reaches $\chi$. 
	\item By Lemma~\ref{synint} we have that $\sem{L}_{k,k} \confcomp \sem{C}_{k,k}$ reaches $\chi$.
	\item By bisimilarity (Lemma~\ref{bisim}) we have that $\sem{L}_{k,k} \semcomp \sem{C}_{k,k}$ reaches $\chi$.
	\item By definition of semantic composition, we know there are traces $\tau \in \sem{L}_{k,k}$ and $\tau^\bot \in \sem{C}_{k,k}$  such that $\sem{L}_{k,k} \xtwoheadrightarrow{\tau} \chi$.
\end{enumerate}

\paragraph{\bf $(2 \implies 1)$:}
\begin{enumerate}
	\item Consider traces $\tau \in \sem{L}_{k_1,l_1}$ and $\tau^\bot \in \sem{C}_{k_2,l_2}$  such that $\sem{L}_{k_1,l_2} \xtwoheadrightarrow{\tau} \chi$.
	\item By definition of semantic composition we have that $\sem{L}_{k_1,l_1} \semcomp \sem{C}_{k_2,l_2}$ reaches $\chi$.
	\item By bisimilarity (Lemma~\ref{bisim}) we have that $\sem{L}_{k_1,l_1} \confcomp \sem{C}_{k_2,l_2}$ reaches $\chi$.
	\item By Lemma~\ref{intsyn} we know $L\syncomp C$ with bound $k_1 + k_2$ reaches $\chi$. 
\end{enumerate}

\end{proof}
}

{\lemma{\label{intsyn}}{
For all composite semantics configurations $\chi = (M,\vec{R},S,\vec{k},\vec{l})$, if $\chi \twoheadrightarrow (M',\vec{R}',S',\vec{k}',\vec{l}')$ where $M' = v'$ or $M' = E[\assert(0)]$, then $\chi^\circ \twoheadrightarrow (M',R',S',k')$.
\begin{proof}
Let $\chi = (M,\vec{R},S,k_1,k_2,l_1,l_2)$ be a configuration that terminates without reaching the bound. Let $\chi^\circ = (M,R_1 \cup R_2,S,k_1 + k_2)$ be the configuration obtained by translating $\chi$. By induction on the length of the transition sequence of $\chi$, we have the following cases.

\paragraph{\bf Base cases:}
\begin{itemize}
	\item \textbf{Case (value):} If $M = v$, then $(v,\vec{R},S,\vec{k},\vec{l})$ is a zero-step transition. From the operational semantics, we have that $(v,R_1 \cup R_2,S,k_1 + k_2)$ is also a zero-step transition. We thus have that $\chi^\circ$ terminates with an equivalent configuration to $\chi$.
	\item \textbf{Case (violation):} This case is identical to (value) but using $M = \assert(0)$ instead of $M=v$, and $()$ instead of $v$ for the return value.
\end{itemize}

\paragraph{\bf Inductive cases:}
\begin{itemize}
	\item \textbf{Case (assert):} If $M = E[\assert(i)]$ where $i \neq 0$, then \[(E[\assert(i)],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[()],\vec{R},S,\vec{k},\vec{l})\] 
	From the operational semantics, we have
	\[(E[\assert(i)],R_1 \cup R_2,S,k_1 + k_2) \to (E[()],R_1 \cup R_2,S,k_1 + k_2)\] 
	This case holds by the inductive hypothesis on $(E[()],\vec{R},S,\vec{k},\vec{l})$.
	
	\item \textbf{Case (dereference):} Same as (assert), but using $S(r)$ instead of $()$ in the second configuration.
	
	\item \textbf{Case (assign):} Same as (assert), but using $S[r \mapsto v]$ instead of $S$ in the second configuration.
	
	\item \textbf{Case (project):} Same as (assert), but using $v_j$ instead of $()$ in the second configuration.
	
	\item \textbf{Case (plus):} Same as (assert), but using $i$ where $i=i_1 \oplus i_2$ instead of $()$ in the second configuration.
	
	\item \textbf{Case (lambda):} Same as (assert), but using $m$ and $m'$, where $m' = m$ by determinacy of the operational semantics, instead of $()$, and using $\vec{R}[m \mapsto \lambda x.M']_i$ and $(R_1 \cup R_2)[m' \mapsto \lambda x.M']$, where updating the repository is preserved under union, instead of $\vec{R}$ and $R_1 \cup R_2$ in the second configuration.
	
	\item \textbf{Case (cond1):} Same as (assert), but using $M_0$ instead of $()$ in the second configuration.
    
	\item \textbf{Case (cond2):} Same as (assert), but using $M_1$ instead of $()$ in the second configuration.
	
	\item \textbf{Case (let):} Same as (assert), but using $M'\{v/x\}$ instead of $()$ in the second configuration.
	
	\item \textbf{Case (letrec):} Same as (assert), but using $M'\{m/x\}$ and $M'\{m'/x\}$ instead of $()$, where $m'=m$ by determinism of the operational semantics, in the second configuration. As with the (lambda) case, this holds because union preserves repository updates.
    
	\item \textbf{Case (app1):} If $M = E[m^i v]$ where $R_i(m) = \lambda x.M'$, then 
	\begin{align*}
	&(E[m^i v],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[\evalbox{M'\{v/x\}^i}^i],\vec{R},S,\vec{k}-_i 1,\vec{l})
	\end{align*}
	From the operational semantics we have
    \begin{align*}
   	&(E[m v],R_1 \cup R_2,S,k_1 + k_2) \to (E[\evalbox{M'\{v/x\}}],R_1 \cup R_2,S,k_1 + k_2 - 1)
    \end{align*}
    Since $\evalbox{M'\{v/x\}}$ is equivalent to $\evalbox{M'\{v/x\}^i}^i$ with all polarity tags removed, this case holds by the inductive hypothesis as with the previous cases.
	
	\item \textbf{Case (app2):} If $M = E[m^i v]$ where $R_{3-i}(m) = \lambda x.M'$ and $v'$ is a refresh of $v$, then
	\begin{align*}
	(E[m^i v],\vec{R},S,\vec{k},\vec{l}) 
	&\compsemto (E[\evaltag{m^{3-i}v'}{i,l_{3-i}-1}],\vec{R}',S,\vec{k},\vec{l}[l_i \mapsto l_0]-_{3-i} 1) \compsemto \dots
	\end{align*}
	From the operational semantics we have
    \begin{align*}
   	&(E[m v],R_1 \cup R_2,S,k_1 + k_2) \to \dots
    \end{align*}
    Since $\evalbox{M'\{v/x\}}$ is equivalent to $\evaltag{m^{3-i}v'}{i,l_{3-i}-1}$ with all polarity tags removed and because $v',\vec{R}'$ are equivalent to $v,\vec{R}$ under determinism, this case holds by the inductive hypothesis as with the previous cases.

	\item \textbf{Case (ret1):} If $M = E[\evalbox{v}^i]$, then
	\begin{align*}
	&(E[\evalbox{v}^i],\vec{R},S,\vec{k},\vec{l}) 
	\compsemto(E[v^i],\vec{R},S,\vec{k}+_i 1,\vec{l})
	\end{align*}
	From the operational semantics we have
	\begin{align*}
	&(E[\evalbox{v}],R_1 \cup R_2,S,k_1 + k_2) \to (E[v],R_1 \cup R_2,S,k_1 + k_2 + 1)
	\end{align*}
	As with the previous case, this case holds by the inductive hypothesis since $v$ is equivalent to $v^i$ without polarity tags.

	\item \textbf{Case (ret2):} If $M = E[\evaltag{v}{i,l}]$, then 
	\begin{align*}
	&(E[\evaltag{v}{i,l}],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[\evalbox{v'}],\vec{R},S,\vec{k},\vec{l}[l_{3-i} \mapsto l, l_i \mapsto last(E)])
	\end{align*}
	From the operational semantics we have
	\begin{align*}
	&(E[\evalbox{v}],R_1 \cup R_2,S,k_1 + k_2)
	\end{align*}
	This case holds by the same reasoning used in the (app2) case.
\end{itemize}
With all cases done, we have that the semantics of $\chi^\circ$ can be obtained from $chi$ if $chi$ terminates without reaching the bound.
\end{proof}
}}

{\lemma{\label{synint}}{
For all composite semantics configurations $\chi = (M,\vec{R},S,\vec{k},\vec{l})$, if $\chi^\circ \twoheadrightarrow (M',R',S',k')$ where $M' = v'$ or $M' = E[\assert(0)]$, then $\chi \twoheadrightarrow (M',\vec{R}',S',\vec{k}',\vec{l}')$.
\begin{proof}
Let $\chi^\circ = (M,R_1\cup R_2,S,k_1 + k_2)$ be a configuration that terminates without reaching the bound. Let $\chi = (M,\vec{R},S,\vec{k},\vec{l})$ where $\vec{l} = l,l$ and $l$ is equal to the number of transition steps left to terminate.
\paragraph{\bf Base cases:}
\begin{itemize}
	\item \textbf{Case (value):} If $M = v$, then $(v,R_1 \cup R_2,S,k_1 + k_2)$ is a zero-step transition. From the composite semantics, we have that $(v,\vec{R},S,k_1,k_2,l,l)$ is also a zero-step transition. We thus have that the semantics of $chi$ can be obtained from $\chi^\circ$.
	\item \textbf{Case (violation):} same as above but with $M = \assert(0)$.
\end{itemize}

\paragraph{\bf Inductive cases:}
\begin{itemize}
	\item \textbf{Case (assert):} If $M = E[\assert(i)]$ where $i \neq 0$, then 	\[(E[\assert(i)],R_1 \cup R_2,S,k_1 + k_2) \to (E[()],R_1 \cup R_2,S,k_1 + k_2)\] 
	From the composite semantics, we have
    \[(E[\assert(i)],\vec{R},S,k_1,k_2,l,l) \compsemto (E[()],\vec{R},S,k_1,k_2,l,l)\] 
	This case holds by the inductive hypothesis on $(E[()],R_1 \cup R_2,S,k_1 + k_2)$, and since bound $\vec{l}$ is big enough to reach a terminal configuration by assumption.
	
	\item \textbf{Case (dereference), (assign), (project), (plus), (lambda), (cond1), (cond2), (let), and (letrec):} As with Lemma~\ref{intsyn}, these cases are identical to (assert) with their corresponding transitions.
    
	\item \textbf{Case (app1):} If $M = E[m^i v]$ where $R_i(m) = \lambda x.M'$, then we have the following equivalent translation into the operational semantics
    \begin{align*}
   	&(E[m v],R_1 \cup R_2,S,k_1 + k_2) \to (E[\evalbox{M'\{v/x\}}],R_1 \cup R_2,S,k_1 + k_2 - 1)
    \end{align*}
	From the composite semantics we have
	\begin{align*}
	&(E[m^i v],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[\evalbox{M'\{v/x\}^i}^i],\vec{R},S,\vec{k}-_i 1,\vec{l})
	\end{align*}
    This case holds by the inductive hypothesis on $(E[\evalbox{M'\{v/x\}}],R_1 \cup R_2,S,k_1 + k_2 - 1)$ since $\vec{l}$ is big enough to reach a terminal configuration by assumption.
	
	\item \textbf{Case (app2):} If $M = E[m^i v]$ where $R_{3-i}(m) = \lambda x.M'$ and $v'$ is a refresh of $v$, then the equivalent operational semantics is
    \begin{align*}
   	&(E[m v],R_1 \cup R_2,S,k_1 + k_2) \to (E[M'\{v/x\}],R_1 \cup R_2,S,k_1 + k_2)
    \end{align*}
	From the composite semantics we have
	\begin{align*}
	&(E[m^i v],\vec{R},S,\vec{k},\vec{l}) \\
	&\compsemto (E[\evaltag{m^{3-i}v'}{i,l_{3-i}-1}],\vec{R}',S,\vec{k},\vec{l}[l_i \mapsto l_0]-_{3-i} 1) \\
    &\compsemto (E[\evaltag{M'{v'/x}^{3-i}}{i,l_{3-i}-1}],\vec{R}',S,\vec{k}-_{3-i} 1,\vec{l}[l_i \mapsto l_0]-_{3-i} 1)
	\end{align*}
    By the same reasoning used for (app1), this case holds by the inductive hypothesis, since $E[M'\{v/x\}]$ is equivalent to $E[\evaltag{M'{v'/x}^{3-i}}{i,l_{3-i}-1}]$ with all polarity tags removed, and because $l$ was originally big enough to reach a terminal configuration by assumption.\todo{proof of tighter $l$ instead of using transition size}

	\item \textbf{Case (ret1):} If $M = E[\evalbox{v}^i]$, then we have
    \begin{align*}
	&(E[\evalbox{v}],R_1 \cup R_2,S,k_1 + k_2) \to (E[v],R_1 \cup R_2,S,k_1 + k_2)
	\end{align*}
	From the composite semantics we have
    \begin{align*}
	&(E[\evalbox{v}^i],\vec{R},S,\vec{k},\vec{l}) 
	\compsemto(E[v^i],\vec{R},S,\vec{k}+_i 1,\vec{l})
	\end{align*}
	By the inductive hypothesis on $(E[v],R_1 \cup R_2,S,k_1 + k_2 + 1)$, we have that $(E[v^i],\vec{R},S,\vec{k}+_i 1,\vec{l})$ terminates with the same value or an assertion violation.
    
	\item \textbf{Case (ret2):} If $M = E[\evaltag{v}{i,l}]$, then we have
	\begin{align*}
	&(E[\evalbox{v}],R_1 \cup R_2,S,k_1 + k_2)
	\end{align*}
	From the composite semantics we have
	\begin{align*}
	&(E[\evaltag{v}{i,l}],\vec{R},S,\vec{k},\vec{l}) \compsemto (E[\evalbox{v'}],\vec{R},S,\vec{k},\vec{l}[l_{3-i} \mapsto l, l_i \mapsto last(E)])
	\end{align*}
	This case holds by the same reasoning used in the (app2) case, and because, to reach this point, $last(E)$ must have been large enough to reach a terminal configuration by assumption.
\end{itemize}
\end{proof}
}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:



==> S-biblio.tex <==
\begin{thebibliography}{10}

\bibitem{AGS2}
  S.~Abramsky, D.~R.~Ghica, A.~S.~Murawski, and C.-H.~L.~Ong. Algorithmic game semantics and component-based verification.
  \newblock In Proc. SAVBCS, 2003.

\bibitem{GS}
S.~Abramsky and G.~McCusker.
\newblock Game Semantics.
\newblock In {\em Logic and Computation}, 1998.
  
\bibitem{smart:surveyAttacks}
N.~Atzei, M.~Bartoletti, and T.~Cimoli.
\newblock A survey of attacks on ethereum smart contracts {S}o{K}.
\newblock In {POST} 2017.

\bibitem{DBLP:conf/cav/BiereCRZ99}
A.~Biere, E.~M. Clarke, R.~Raimi, and Y.~Zhu.
\newblock Verifiying safety properties of a power {PC} microprocessor using
  symbolic model checking without {BDD}s.
\newblock In Proc.~{CAV} 1999.

\bibitem{symbolic:select}
R.~S.~Boyer, B.~Elspas, and K.~Levitt.^
\newblock Select—a formal system for testing and debugging programs by
  symbolic execution.
\newblock In Proc. International Conference on Reliable Software, 1975.

\bibitem{klee}
C.~Cadar, D.~Dunbar, and D.~Engler.
\newblock Klee: Unassisted and automatic generation of high-coverage tests for
  complex systems programs.
\newblock In Proc. {OSDI} 2008.

\bibitem{DBLP:conf/tacas/ClarkeKL04}
E.~M. Clarke, D.~Kroening, and F.~Lerda.
\newblock A tool for checking {ANSI-C} programs.
\newblock In Proc. {TACAS} 2004.

\bibitem{Clarke:ModelChecking}
E.~M. Clarke, Jr., O.~Grumberg, and D.~A. Peled.
\newblock {\em Model Checking}.
\newblock MIT Press, Cambridge, MA, USA, 1999.

\bibitem{z3}
L.~M. de~Moura and N.~Bj{\o}rner.
\newblock {Z3:} an efficient {SMT} solver.
\newblock In {TACAS} 2008.

\bibitem{Dimovski}
A.~S.~Dimovski.
\newblock Program verification using symbolic game semantics.
\newblock TCS, 2014.

\bibitem{survey:verification}
V.~D'Silva, D.~Kroening, and G.~Weissenbacher.
\newblock A survey of automated techniques for formal software verification.
\newblock {IEEE TCAD}, 2008.

\bibitem{dao}
Q.~Dupont.
\newblock {\em Experiments in Algorithmic Governance: A history and ethnography
  of " The DAO, " a failed Decentralized Autonomous Organization}.
\newblock Routledge, 2017.

\bibitem{symbolic:dissect}
W.~E.~Howden.
\newblock Symbolic testing and the dissect symbolic evaluation system.
\newblock {IEEE TSE}, 1977.

\bibitem{GS2}
D.~R.~Ghica.
\newblock Applications of game semantics: from program analysis to hardware synthesis.
\newblock In Proc. LICS 2009.

\bibitem{AGS1}
  D.~R.~Ghica and G.~McCusker.
  \newblock Reasoning about Idealized Algol using regular expressions.
  \newblock In Proc. ICALP 2000.

\bibitem{OGS3}
D.~R. Ghica and N.~Tzevelekos.
\newblock A system-level game semantics.
\newblock {ENTCS}, 2012.

\bibitem{partial:order:1}
P.~Godefroid.
\newblock {\em Partial-Order Methods for the Verification of Concurrent
  Systems: An Approach to the State-Explosion Problem}.
\newblock Springer-Verlag, 1996.

\bibitem{smart:foundationsTools}
I.~Grishchenko, M.~Maffei, and C.~Schneidewind.
\newblock Foundations and tools for the static analysis of Ethereum smart
  contracts.
\newblock In Proc. {CAV} 2018.

\bibitem{OGS1}
A.~{Jeffrey} and J.~{Rathke}.
\newblock A fully abstract may testing semantics for concurrent objects.
\newblock In Proc. {LICS} 2002.

\bibitem{symbolic:king}
J.~King.
\newblock A new approach to program testing.
\newblock In Proc. International Conference on Reliable Software, 1975.

\bibitem{cprover:cbmc}
D.~Kroening.
\newblock The cbmc homepage.
\newblock \url{http://www.cprover.org/cbmc/}, 2017.
%\newblock [Online; accessed 20-Jun-2019].

\bibitem{OGS2}
J.~Laird.
\newblock A fully abstract trace semantics for general references.
\newblock In {ICALP} 2007.

\bibitem{smart:reguard}
C.~{Liu}, H.~{Liu}, Z.~{Cao}, Z.~{Chen}, B.~{Chen}, and B.~{Roscoe}.
\newblock Reguard: Finding reentrancy bugs in smart contracts.
\newblock In Proc. {ICSE} 2018.

\bibitem{smart:oyente}
L.~Luu, D.-H. Chu, H.~Olickel, P.~Saxena, and A.~Hobor.
\newblock Making smart contracts smarter.
\newblock In Proc. CCS, 2016.

\bibitem{DBLP:conf/tacas/MorseRCN014}
J.~Morse, M.~Ramalho, L.~C. Cordeiro, D.~Nicole, and B.~Fischer.
\newblock {ESBMC} 1.22 - (competition contribution).
\newblock In Proc. {TACAS} 2014.

\bibitem{coneqct}
A.~S.~Murawski, S.~J.~Ramsay, and N.~Tzevelekos.
\newblock A contextual equivalence checker for {IMJ}*.
\newblock In Proc. {ATVA} 2015.

\bibitem{mochi}
R.~Sato, H.~Unno, and N.~Kobayashi.
\newblock Towards a scalable software model checker for higher-order programs.
\newblock {PEPM} 2013.

\bibitem{DBLP:journals/corr/MurawskiT16a}
A.~S. Murawski and N.~Tzevelekos.
\newblock Higher-order linearisability.
\newblock JLAMP, 2019.

\bibitem{smart:majan}
I.~Nikoli\'{c}, A.~Kolluri, I.~Sergey, P.~Saxena, and A.~Hobor.
\newblock Finding the greedy, prodigal, and suicidal contracts at scale.
\newblock In Proc. {ACSAC} 2018.

\bibitem{bmc:concurrent}
Q.~Phan, P.~Malacaria, and C.~S. Pasareanu.
\newblock Concurrent bounded model checking.
\newblock {ACM} {SIGSOFT} {SEN}, 2015.

\bibitem{nom2}
A.~M. Pitts.
\newblock {\em Nominal Sets: Names and Symmetry in Computer Science}.
\newblock CUP,\,2013.

\bibitem{akward}
A.~M.~Pitts and I.~D.~B.~Stark.
\newblock Operational Reasoning for Functions with Local State.
\newblock {\em Higher Order Operational Techniques in Semantics}, 1998.

\bibitem{k:framework}
G.~Roşu and T.~Şerbănuţă.
\newblock An overview of the K semantic framework.
\newblock {J.LAP},\,2010.

\bibitem{jcute}
K.~Sen and G.~Agha.
\newblock Cute and jcute: Concolic unit testing and explicit path
  model-checking tools.
\newblock In Proc. {CAV} 2006.

\bibitem{fuzzers:vs:symbolic}
I.~Yun, S.~Lee, M.~Xu, Y.~Jang, and T.~Kim.
\newblock Qsym: A practical concolic execution engine tailored for hybrid
  fuzzing.
\newblock In Proc. {SEC} 2018.

\end{thebibliography}


==> S-games.tex <==
\section{Semantics for Open Libraries: bounded, then symbolic}

We define the bounded operational game semantics rules parametrised on bounds $l,k \in \mathbb{N}$, with initial bounds $k_0,l_0 \in \mathbb{N}$, for proponent configurations of the form $(\eval,M,R,\pub,\abs,S,k,-)$ and opponent configurations of the form $(\eval,-,R,\pub,\abs,S,k,l)$. We use $k$ to bound internal moves as in the operational semantics. More subtly, $l$ bounds the number of descendent opponent nodes under a given layer in the symbolic computation tree, which is equivalent to the total number of \textsc{OQ} moves from a given layer of a branch. This means that $l$ bounds the depth and width of the resulting symbolic computation tree.

\todo{mention $l_0$}

\renewcommand{\arraystretch}{1.5}
\begin{tabular}{RLRL}
(\textsc{Int})&
(\eval,M,R,\pub,\abs,S,k,-)
\rightarrow (\eval,M',R',\pub,\abs,S',k',-)
\\&\qquad\text{where }(M,R,S,k)\to^{*}(M',R',S',k')
\\
(\textsc{Pq})&
(\eval,E[mv],R,\pub,\abs,S,k,-)
\xrightarrow{\mathtt{call}(m,v)} (m::E::\eval,-,R,\pub',\abs,S,k,l_0)
\\&\qquad\text{where $m \in \abs$ and (\textbf{PC})}
\\
(\textsc{Oq})&
(\eval,-,R,\pub,\abs,S,k,l+1)
\xrightarrow{\mathtt{call}(m,v)} (l::m::\eval,mv,R,\pub,\abs',S,k,-)
\\&\qquad\text{where $m \in \pub$, $R(m)=\lambda x.M$ and (\textbf{OC})}
\\
(\textsc{Pa})&
(l::m::\eval,v,R,\pub,\abs,S,k,-)
\xrightarrow{\mathtt{ret}(m,v)} (\eval,-,R,\pub',\abs,S,k,l)
\\&\qquad\text{where $m \in \pub$ and (\textbf{PC})}
\\
(\textsc{Oa})&
(m::E::\eval,-,R,\pub,\abs,S,k,l)
\xrightarrow{\mathtt{ret}(m,v)} (\eval,E[v],R,\pub,\abs',S,k,-)
\\&\qquad\text{where $m \in \abs$ and (\textbf{OC})}
\\
\end{tabular}

(\textbf{PC})\quad If $v$ contains $m_1,...,m_n\in\meths$ then $\pub' = \pub \cup \{ m_1, ..., m_n\}$.

(\textbf{OC})\quad
If $v$ contains $m_1,...,m_n\in\meths$ then each $m_i$ is fresh in $dom(R) \uplus \abs$ and appears in $v$ only once, and $\abs' = \abs \cup \{m_1,...,m_n\}$.

\subsection{Bounded Symbolic Game Semantics}
Based on the operational game semantics, we define a labelled transition system corresponding to the small-step symbolic execution of a game between proponent and opponent configurations, where labels indicate the move played to make the transition. For this, we first define the following configurations:
\begin{flalign*}
Proponent\quad &(\eval,M,R,\pub,\abs,\tau,\sigma,pc,k,-)_p\\
Opponent\quad &(\eval,-,R,\pub,\abs,\tau,\sigma,pc,k,l)_o
\end{flalign*}
with evaluation stack $\eval$, proponent term $M$, opponent step bound $l \in \mathbb{N}$, method repository $R$, public and abstract name sets $\pub$ and $\abs$, trace $\tau$ for moves $\mu$, and $\sigma$ and $pc$ as previously.

We now modify our symbolic execution ($\symto$) to make it compatible with games. First, we extend all final configurations by adding the method repository $R$ and the bound $k$ to the triples. This requires updating these base cases:
\begin{flalign*}
&\symext(E[mv],R,\sigma,pc,0) \symto (\nil,R,\sigma,pc,0)\\
&\symext(v,R,\sigma,pc,k) \text{ is a final configuration}\\
&\symext(E[\assert(0)],R,\sigma,pc,k) \symto (\fail,R,\sigma,pc,k)\\
&\symext(E[\assert(x)],R,\sigma,pc,k) \symto (\fail,R,\sigma,pc \land (\sigma(x)\neq 0),k)
\end{flalign*}
We also allow configurations containing $E[mv]$ where $m \nin dom(R)$ to get stuck, thus removing the requirement for free variables of ground type.

We proceed by defining the transition rules ($\gamto$).

\cutout{
Where used, $\mu$ is a variable freshly generated such that $\forall \mu'.\mu'\sqsubset\mu$ if move $\mu'$ occurs before move $\mu$ in some path; i.e. there exists a chronological ordering $\sqsubset$ for $\mu$ and every $\mu$ in a path is unique. We can observe that the following rules build a symbolic execution tree. From any given configuration, every applicable rule is used, each adding a new branch to the tree.}

\todo{mention $l_0$}

\subsection{Proponent Configurations}

\paragraph{Terminal Rules:}
\begin{flalign*}
&(\eval,\nil,R,\pub,\abs,\tau,\sigma,pc,0,-)_p \gamto (\nil,\tau,\sigma,pc)\\
&(\eval,\fail,R,\pub,\abs,\tau,\sigma,pc,k,-)_p \gamto (\fail,\tau,\sigma,pc)\\
&(\varnothing,v,R,\pub,\abs,\tau,\sigma,pc,k,-)_p \gamto (v,\tau,\sigma,pc)
\end{flalign*}

\paragraph{Internal Moves:}
\begin{flalign*}
{\begin{prooftree}
\Hypo{ (M,R,\sigma,pc,k) \symto^* (M',R',\sigma',pc',k')}
\Infer1[]{ (\eval,M,R,\pub,\abs,\tau,\sigma,pc,k,-)_p 
\gamto (\eval,M',R',\pub,\abs,\tau,\sigma',pc',k',-)_p}
\end{prooftree}}
\end{flalign*}

\paragraph{Proponent Question:}
\begin{flalign*}
&(\eval,E[m\tilde v],R,\pub,\abs,\tau,\sigma,pc,k,-)_p \\
&\qquad \xgamto{\mathtt{call}(m,\widetilde{v})}
(m::E::\eval,-,R,\pub',\abs,\tau \cdot \mathtt{call}(m,\widetilde{v}),\sigma,pc,k,l_0)_o\\
&\quad \text{where $m \in \abs$ and (\textbf{PC})}
\end{flalign*}

\paragraph{Proponent Answer:}
\begin{flalign*}
&(l::m::\eval,v,R,\pub,\abs,\tau,\sigma,pc,k,-)_p \\
&\qquad \xgamto{\mathtt{ret}(m,\tilde{v})}
(\eval,-,R',\pub',\abs,\tau\cdot \mathtt{ret}(m,\tilde{v}),\sigma,pc,k,l)_o\\
&\quad \text{where $m \in \pub$ and (\textbf{PC})}
\end{flalign*}

\subsection{Opponent Configurations}
\paragraph{Terminal Rules:}
\begin{flalign*}
&(\eval,-,R,\pub,\abs,\tau,\sigma,pc,k,0)_o \gamto (\nil,\tau,\sigma,pc)\\
\end{flalign*}

\paragraph{Opponent Question:}
\begin{flalign*}
&(\eval,-,R,\pub,\abs,\tau,\sigma,pc,k,l+1)_o \\
&\qquad \xgamto{\mathtt{call}(m,\tilde v)} (l::m::\eval,m\tilde v,R,\pub,\abs',\tau\cdot \mathtt{call}(m,\tilde v),\sigma,pc,k,-)_p\\
&\quad \text{where $m \in \pub$ and (\textbf{OC})}
\end{flalign*}

\paragraph{Opponent Answer:}
\begin{flalign*}
&(m::E::\eval,-,R,\pub,\abs,\tau,\sigma,pc,k,l)_o \\
&\qquad \xgamto{\mathtt{ret}(m,\tilde v)} (\eval,E[\tilde v],R,\pub,\abs',\tau\cdot \mathtt{ret}(m,\tilde v),\sigma,pc,k,-)_p\\
&\quad \text{where $m \in \pub$ and (\textbf{OC})}
\end{flalign*}

(\textbf{PC})\quad If $\tilde v$ contains method names $m_1,...,m_n$ then
$\pub' = \pub \cup \{ m_1, ..., m_n\}$.

(\textbf{OC})\quad $(\tilde v,\abs')=f(\theta,\abs)$, where $\theta$ is the expected type  of $\tilde v$ and: \begin{align*}
&f(\theta,\abs) = 
\begin{cases} 
((),\abs) & \text{if $\theta = \mathtt{unit}$}\\
(\kappa,\abs\uplus\{\kappa\}) & \text{if $\theta = \mathtt{int}$, and $\kappa$ is fresh in $dom(\sigma) \uplus \abs$}\\
(m,\abs\uplus\{m\}) & \text{if $\theta = \tau \to \tau'$, and $m$ is fresh in $dom(R) \uplus \abs$}\\
(\pair{\tilde v_1, \tilde v_2},\abs_2) & \text{if $\theta = \tau_1 \times \tau_2$ and }
f(\tau_1,\abs)=(\tilde v_1,\abs_1), f(\tau_2,\abs_1)=(\tilde v_2,\abs_2)
\end{cases}
\end{align*}

Note that we are using $o$ and $p$ to tag the \boldemph{polarity} of configurations, by which we mean that they are opponent and proponent configurations respectively. We will also use this polarity to describe moves; moves of polarity $X \in \{o,p\}$ ($X$-moves) are played from an $X$-configuration. 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


